An Asymptotically Optimal Approximation of the Conditional Mean Channel Estimator based on Gaussian Mixture Models

This paper investigates a channel estimator based on Gaussian mixture models (GMMs). We fit a GMM to given channel samples to obtain an analytic probability density function (PDF) which approximates the true channel PDF. Then, a conditional mean channel estimator corresponding to this approximating PDF is computed in closed form and used as an approximation of the optimal conditional mean estimator based on the true channel PDF. This optimal estimator cannot be calculated analytically because the true channel PDF is generally not available. To motivate the GMM-based estimator, we show that it converges to the optimal conditional mean estimator as the number of GMM components is increased. In numerical experiments, a reasonable number of GMM components already shows promising estimation results.

==> Definitions/LaTeXMacrosOld.tex <==
% last update: 28. November 2003

% text commands
%\newcommand{\comment}[1]{}
\newcommand{\quotes}[1]{\glqq{#1}\grqq}
%\newcommand{\Definition}[1]{{\bfseries Definition: \quad}\emph{#1}}
\newcommand{\Remark}[1]{{\bfseries Achtung: \quad}{#1}}
\newcommand{\Special}[1]{{\bfseries Spezialfall: \quad}{#1}}

% logical and arithmetical symbols
\newcommand{\defequalto}{\stackrel{\mbox{\scriptsize$\triangle$}}{=}}
%\newcommand{\C}{{\operatorname{c}}}

% sets and spaces
\newcommand{\DefSet}[1]{\mathcal{#1}}
\newcommand{\DefSpace}[1]{\mathbb{#1}}

\newcommand{\SetA}{\mathcal{A}}
\newcommand{\SetB}{\mathcal{B}}
\newcommand{\SetI}{\mathcal{I}}

\newcommand{\SpaceB}{\mathbb{B}}
\newcommand{\SpaceC}{\mathbb{C}}
\newcommand{\SpaceF}{\mathbb{F}}
\newcommand{\SpaceJ}{\mathbb{J}}
\newcommand{\SpaceN}{\mathbb{N}}
\newcommand{\SpaceP}{\mathbb{P}}
\newcommand{\SpaceQ}{\mathbb{Q}}
\newcommand{\SpaceR}{\mathbb{R}}
\newcommand{\SpaceS}{\mathbb{S}}
\newcommand{\SpaceZ}{\mathbb{Z}}
\newcommand{\SpaceG}{\mathbb{G}}
\newcommand{\SpaceU}{\mathbb{U}}
\newcommand{\SpaceV}{\mathbb{V}}
\newcommand{\SpaceX}{\mathbb{X}}
\newcommand{\SpaceY}{\mathbb{Y}}
\newcommand{\SpaceT}{\mathbb{T}}

% vectorspaces
\newcommand{\metric}[1]{\operatorname{d}\!\left(#1\right)}
\newcommand{\norm}[1]{\left\|#1\right\|}
\newcommand{\normP}[1]{{\left\|#1\right\|}_{\SpaceOf{P}}}
\newcommand{\iprod}[1]{{\left\langle#1\right\rangle}}
\newcommand{\iprodP}[1]{{\left\langle#1\right\rangle}_{\SpaceOf{P}}}

% operators
\newcommand{\Op}[1]{{\operatorname{#1}}}
\newcommand{\Opbar}[1]{{\bar{\operatorname{#1}}}}
\newcommand{\Id}{{\operatorname{Id}}}

% vectors, matrices
%\newcommand{\B}[1]{\boldsymbol{#1}}
\newcommand{\Bhat}[1]{\boldsymbol{\hat{#1}}}
\newcommand{\Bhathat}[1]{\boldsymbol{\hat{\hat{#1}}}}
\newcommand{\Bbar}[1]{\boldsymbol{\bar{#1}}}
\newcommand{\Btilde}[1]{\boldsymbol{\tilde{#1}}}
\newcommand{\Bbreve}[1]{\boldsymbol{\breve{#1}}}
\newcommand{\Vector}[1]{\operatorname{vec}\left[#1\right]}

\newcommand{\Tr}{{\operatorname{T}}}
\newcommand{\He}{{\operatorname{H}}}
\newcommand{\Ad}{{\operatorname{A}}}

\newcommand{\Trace}[1]{\operatorname{tr}\left[#1\right]}
\newcommand{\Diag}[1]{\operatorname{diag}\left[#1\right]}
\newcommand{\Rank}[1]{\operatorname{rank}\left[#1\right]}
\newcommand{\Dim}[1]{\operatorname{dim}\left[#1\right]}
\newcommand{\Null}[1]{\operatorname{null}\left[#1\right]}
\newcommand{\Span}[1]{\operatorname{span}\left[#1\right]}
\newcommand{\Basis}[1]{\operatorname{basis}\left[#1\right]}
\newcommand{\Range}[1]{\operatorname{range}\left[#1\right]}

% functions
\newcommand{\rectfunc}[1]{\operatorname{rect}\left(#1\right)}
\newcommand{\sinc}[1]{\operatorname{sinc}\left(#1\right)}
\newcommand{\e}{\operatorname{e}}
\newcommand{\rect}[1]{\operatorname{rect}\left(#1\right)}

% complex number
\renewcommand{\j}{\operatorname{j}}
\newcommand{\Real}[1]{\operatorname{Re}\left\{#1\right\}}
\newcommand{\Imag}[1]{\operatorname{Im}\left\{#1\right\}}
\newcommand{\unit}{\operatorname{unit}}

% infinitesimal calculus
\newcommand{\diff}{\operatorname{d}\!}
\newcommand{\dt}{\operatorname{d}\!t}
\newcommand{\dx}{\operatorname{d}\!x}
\newcommand{\dy}{\operatorname{d}\!y}
\newcommand{\dz}{\operatorname{d}\!z}
\newcommand{\dtau}{\operatorname{d}\!\tau}
\newcommand{\dxi}{\operatorname{d}\!\xi}
\newcommand{\df}{\operatorname{d}\!f}
\newcommand{\dP}{\operatorname{d}\!P}
\newcommand{\PartialDerivative}[2]{\frac{\partial #1}{\partial #2}}

% optimization
%\newcommand{\argmin}{\operatorname{arg}\!\min}
%\newcommand{\argmax}{\operatorname{arg}\!\max}
\newcommand{\st}{\quad\text{\sf s. t.}\quad}
\newcommand{\udN}{\quad\text{\sf u. d. N.}\quad}

% random variables
\DeclareMathAlphabet{\mathss}{T1}{cmss}{m}{sl}
\newcommand{\rv}[1]{{\mathss #1}}
\DeclareMathAlphabet{\mathbss}{T1}{cmss}{bx}{sl}
\newcommand{\Brv}[1]{{\mathbss #1}}
\newcommand{\hatrv}[1]{\hat{\rv #1}}
\newcommand{\tilrv}[1]{\tilde{\rv #1}}
\newcommand{\barrv}[1]{\bar{\rv #1}}
%\newcommand{\Brv}[1]{{\boldsymbol{\rv #1}}}
\newcommand{\Bhatrv}[1]{\hat{\Brv #1}}
\newcommand{\Bhathatrv}[1]{\boldsymbol{\hat{\hat{\rv #1}}}}
\newcommand{\Bbarrv}[1]{\boldsymbol{\bar{\rv #1}}}
\newcommand{\Btilrv}[1]{\boldsymbol{\tilde{\rv #1}}}

% stochastic operators
\newcommand{\Normal}[1]{\operatorname{N}\left(#1\right)}
\newcommand{\Exp}[1]{\operatorname{E}\left[#1\right]}
\newcommand{\Expe}[2]{\operatorname{E}_{#1}\left[#2\right]}
\newcommand{\Var}[1]{\operatorname{Var}\left[#1\right]}
\newcommand{\Vari}[2]{\operatorname{Var}_{#1}\left[#2\right]}
\newcommand{\Cov}[2]{\operatorname{Cov}\left[#1,#2\right]}
\newcommand{\CovC}[3]{\operatorname{Cov}_{#1}\left[#2,#3\right]}
\newcommand{\Pof}[1]{\operatorname{P}\left(#1\right)}
\newcommand{\Pofrv}[2]{\operatorname{P}_{#1}\left(#2\right)}
\newcommand{\Pofif}[2]{\operatorname{P}_{#2}\left(#1\right)}
\newcommand{\rvalpha}{{\alpha}}
\newcommand{\rveta}{{\eta}}
\newcommand{\Brveta}{{\B\eta}}

% abbreviations
\newcommand{\ges}{\text{\sf ges}}
\newcommand{\fo}{f_{\text{\sf 0}}}
\newcommand{\To}{T_{\text{\sf 0}}}
\newcommand{\fa}{f_{\text{\sf a}}}
\newcommand{\Ta}{T_{\text{\sf a}}}
\newcommand{\Tp}{T_{\text{\sf p}}}
\newcommand{\Ts}{T_{\text{\sf s}}}
\newcommand{\pc}{p_{\text{\sf c}}}
\newcommand{\cyc}{\text{\sf c}}
\newcommand{\fG}{f_{\text{\sf G}}}
\newcommand{\TG}{T_{\text{\sf G}}}
\newcommand{\Ns}{N_{\text{\sf s}}}
\newcommand{\Np}{N_{\text{\sf p}}}

% MIMO systems
\newcommand{\Rx}{\text{\sf Rx}}
\newcommand{\Tx}{\text{\sf Tx}}
\newcommand{\MRx}{{M_{\text{\sf R}}}}
\newcommand{\MTx}{{M_{\text{\sf T}}}}

\newcommand{\BH}{\B H}
\newcommand{\BG}{\B G}
\newcommand{\BGMF}{\B G_{\text{\sf RxMF}}}
\newcommand{\BGZF}{\B G_{\text{\sf RxZF}}}
\newcommand{\BGWF}{\B G_{\text{\sf RxWF}}}
\newcommand{\BP}{\B P}
\newcommand{\BPMF}{\B P_{\text{\sf TxMF}}}
\newcommand{\BPZF}{\B P_{\text{\sf TxZF}}}
\newcommand{\BPWF}{\B P_{\text{\sf TxWF}}}

\newcommand{\BRxx}{\B C_{\rv x,\rv x}}
\newcommand{\BRyy}{\B C_{\rv y,\rv y}}
\newcommand{\BbarRyy}{\B C_{\barrv y,\barrv y}}
\newcommand{\BRss}{\B C_{\rv s,\rv s}}
\newcommand{\BRnn}{\B C_{\rveta,\rveta}}
\newcommand{\BbarRnn}{{\B C_{\bar{\rveta},\bar{\rveta}}}}
\newcommand{\BRhh}{\B C_{\rv h,\rv h}}
\newcommand{\BRHH}{\B C_{\rv H,\rv H}}
\newcommand{\BhatRHH}{\Bhat C_{\rv H,\rv H}}

\newcommand{\BRxs}{\B C_{\rv x,\rv s}}
\newcommand{\BRsx}{\B C_{\rv s,\rv x}}
\newcommand{\BRsn}{\B C_{\rv s,\rveta}}
\newcommand{\BRns}{\B C_{\rveta,\rv s}}
\newcommand{\BRhy}{\B C_{\rv h,\rv y}}
\newcommand{\BbarRhy}{\B C_{\barrv h,\barrv y}}

\newcommand{\MSE}{\varepsilon_{\text{\sf MSE}}}
\newcommand{\ssquare}{\sigma_{\rv s}^2}
\newcommand{\nsquare}{\sigma_{\rv n}^2}
\newcommand{\overssquare}{\sigma_{\rv s}^{-2}}
\newcommand{\overnsquare}{\sigma_{\rv n}^{-2}}

\newcommand{\LP}{{\text{\sf LP}}}
\newcommand{\LS}{{\text{\sf LS}}}
\newcommand{\MLE}{{\text{\sf ML}}}
\newcommand{\MS}{{\text{\sf MSE}}}
\newcommand{\WF}{{\text{\sf WF}}}

% definecolor 
\definecolor{red}{rgb}{0.98,0.75,0.25}          % #fa1340
\definecolor{green4}{rgb}{0,0.57,0}             % #009000
\definecolor{blue4}{rgb}{0,0,0.57}              % #000090
\definecolor{Ltblue}{rgb}{0.53,0.81,1}          % #87ceff
\definecolor{red4}{rgb}{0.57,0,0}               % #900000
\definecolor{bg_green}{rgb}{0.85,1,0.85}        % #d9ffd9
\definecolor{bg_blue}{rgb}{0.85,0.85,1}         % #d9d9ff
\definecolor{bg_red}{rgb}{1,0.85,0.85}          % #ffd9d9
\definecolor{bg_yellow}{rgb}{1,1,0.44}          % #ffff70
\definecolor{gold}{rgb}{1,0.90,0}               % #ffd700

% SSV Skript
\newcommand{\detbrack}[1]{\operatorname{det}\left(#1\right)}
\newcommand{\comp}{\operatorname{\mathsf{C}}}
\newcommand{\dOmega}{\mathsf{\Omega}}
%\DeclareMathOperator{\comp}{C}
\DeclareMathOperator{\expectop}{E}
\DeclareMathOperator{\varop}{Var}
\DeclareMathOperator{\bias}{Bias}
\DeclareMathOperator{\expectopd}{E}
\DeclareMathOperator{\varopd}{Var}
\DeclareMathOperator{\covop}{Cov}
\DeclareMathOperator{\traceop}{tr}
%\newcommand{\tr}[1]{\traceop \left[#1\right]}
\newcommand{\expect}[1]{\expectop\left[#1\right]}
\newcommand{\expectd}[2]{\expectop\left[#1\right]}
\newcommand{\variance}[1]{\varop\left[#1\right]}
\newcommand{\varianced}[2]{\varop\left[#1\right]}
\newcommand{\cov}[1]{\covop\left[#1\right]}
\newcommand{\fnccorr}[2]{r_{#1}\left(#2\right)}
%\newcommand{\fnccorr}[2]{r_{#1}\left[#2\right]}
\newcommand{\fnccov}[2]{c_{#1}\left[#2\right]}
\newcommand{\lds}[2]{S_{#1}\left(#2\right)}
\newcommand{\trace}[1]{\textrm{tr}\left[#1\right]}

%\renewcommand{\labelenumi}{\alph{enumi})}
%\renewcommand{\labelenumii}{\arabic{enumii})}

\newcommand{\ergebnis}{\mathcal{A}}
\newcommand{\ergebnisb}{\mathcal{B}}

\newcommand{\bs}{\boldsymbol}
\newcommand{\transpose}{\mathrm{T}}
\newcommand{\hermit}{\mathrm{H}}
\newcommand{\nrvsymbol}{N}
\newcommand{\nrv}{\random{\nrvsymbol}}
\newcommand{\nrvv}{\Brandom{\nrvsymbol}}
\newcommand{\vrvsymbol}{v}
\newcommand{\vrv}{\random{\vrvsymbol}}
\newcommand{\vrvv}{\Brandom{\vrvsymbol}}
\newcommand{\xrvsymbol}{X}
\newcommand{\xrv}{\random{\xrvsymbol}}
\newcommand{\xrvv}{\Brandom{\xrvsymbol}}
\newcommand{\yrvsymbol}{Y}
\newcommand{\yrv}{\random{\yrvsymbol}}
\newcommand{\yrvv}{\Brandom{\yrvsymbol}}
\newcommand{\zrvsymbol}{Z}
\newcommand{\zrv}{\random{\zrvsymbol}}
\newcommand{\zrvv}{\Brandom{\zrvsymbol}}
\newcommand{\arvsymbol}{A}
\newcommand{\arv}{\random{\arvsymbol}}
\newcommand{\brvsymbol}{B}
\newcommand{\brv}{\random{\brvsymbol}}
\newcommand{\srvsymbol}{S}
\newcommand{\srv}{\random{\srvsymbol}}
\newcommand{\srvv}{\Brandom{\srvsymbol}}
\newcommand{\htt}{\hat\theta}
\newcommand{\cdf}[2]{F_{#1}(#2)}
\newcommand{\pdf}[2]{f_{#1}(#2)}
\newcommand{\prob}[1]{P\left(#1\right)}
\newcommand{\probd}[2]{P_{#1}\left(#2\right)}
\newcommand{\nx}{\xrv_{1},\ldots,\xrv_{N}}
\newcommand{\nxr}{x_{1},\ldots,x_{N}}
%\newcommand{\NN}{\text{N}}
%\renewcommand{\thefootnote}{\fnsymbol{footnote}}
%\newcommand{\eye}{\boldsymbol{I}}
\newcommand{\hea}[1]{\noindent\textsf{\textbf{#1}}}

%\newcommand{\argmin}[2]{{\underset{#1}{\textrm{argmin}}\left\{#2\right\}}}
%\newcommand{\argmax}[2]{{\underset{#1}{\textrm{argmax}}\left\{#2\right\}}}
\newcommand{\est}[1]{T_{#1}}
\newcommand{\estr}[1]{\random{T}_{#1}}
%\newcommand{\Def}{\noindent \underline{\textbf{Def.:}}\quad}
%\newcommand{\Def}{\noindent $\rightarrow$ \quad}
\newcommand{\Def}{}
\newcommand{\Stat}{\{\mathbb{X},\,\mathbb{F},\,\textrm{P}_{\bs{\theta}}; \,
    \bs{\theta}\in\bs{\Theta}\}}
\newcommand{\Stats}{\{\mathbb{X},\,\mathbb{F},\,\textrm{P}_{\theta}; \,
    \theta\in\Theta\}}
\newcommand{\ML}{\text{L}(x;\theta)}
\newcommand{\MLr}{\text{L}(\xrv;\theta)}
\newcommand{\MLi}{\text{L}(x_i;\theta)}
\newcommand{\MLnx}{\text{L}(\nxr;\theta)}
\newcommand{\MLv}{\text{L}(\bs{x};\theta)}
\newcommand{\bML}{\text{L}(\xrv;\bs{\theta})}
\newcommand{\bMLi}{\text{L}(\xrv_i;\bs{\theta})}
\newcommand{\bMLnx}{\text{L}(\nx;\bs{\theta})}
\newcommand{\bMLv}{\text{L}(\xrvv;\bs{\theta})}
\newcommand{\bMLr}{\text{L}(x;\bs{\theta})}
\newcommand{\bMLir}{\text{L}(x_i;\bs{\theta})}
\newcommand{\bMLnxr}{\text{L}(\nxr;\bs{\theta})}
\newcommand{\bMLvr}{\text{L}(\bs{x};\bs{\theta})}
\newcommand{\TML}{T_{\text{ML}}}
\newcommand{\BBB}{\newpage\noindent}
\newcommand{\gs}{g(x,\theta)}
\newcommand{\gsr}{g(\xrv,\theta)}
\newcommand{\WDF}{Wahrscheinlichkeitsdichtefunktion }
\newcommand{\BRE}{\par\vspace{0.5cm}\noindent}
\newcommand{\rmnum}[1]{\romannumeral #1}
\newcommand{\Rmnum}[1]{\expandafter\@slowromancap\romannumeral #1@}
\newcommand{\GDN}{G_d(\theta)\vert_{\theta \in \Theta_0}}
\newcommand{\GDA}{G_d(\theta)\vert_{\theta \in \Theta_1}}
\newcommand{\LQ}{\frac{\pdf{\xrv}{x; \theta_1}}{\pdf{\xrv}{x; \theta_0}}}

